Predictor Selection for Synthetic Controls

Synthetic control methods often rely on matching pre-treatment characteristics (called predictors) of the treated unit. The choice of predictors and how they are weighted plays a key role in the performance and interpretability of synthetic control estimators. This paper proposes the use of a sparse synthetic control procedure that penalizes the number of predictors used in generating the counterfactual to select the most important predictors. We derive, in a linear factor model framework, a new model selection consistency result and show that the penalized procedure has a faster mean squared error convergence rate. Through a simulation study, we then show that the sparse synthetic control achieves lower bias and has better post-treatment performance than the un-penalized synthetic control. Finally, we apply the method to revisit the study of the passage of Proposition 99 in California in an augmented setting with a large number of predictors available.

==> paper_tables/top7_predictors.tex <==
\begin{tabular}{ll}
\toprule
                      SCM &       \textit{Sparse} SCM \\
\midrule
                  smk\_80 &          smk\_75 \\
     general\_revenue\_inc &   incshare\_top1 \\
                  smk\_75 &          smk\_88 \\
                  smk\_88 &      pc\_inc\_ann \\
                  loginc &          region \\
 general\_expenditure\_inc &  budget\_surplus \\
              pc\_inc\_ann &       taxes\_gsp \\
\bottomrule
\end{tabular}

